Coordinated Dynamic Spectrum Management of LTE-U and Wi-Fi Networks

This paper investigates the co-existence of Wi-Fi and LTE in emerging unlicensed frequency bands which are intended to accommodate multiple radio access technologies. Wi-Fi and LTE are the two most prominent access technologies being deployed today, motivating further study of the inter-system interference arising in such shared spectrum scenarios as well as possible techniques for enabling improved co-existence. An analytical model for evaluating the baseline performance of co-existing Wi-Fi and LTE is developed and used to obtain baseline performance measures. The results show that both Wi-Fi and LTE networks cause significant interference to each other and that the degradation is dependent on a number of factors such as power levels and physical topology. The model-based results are partially validated via experimental evaluations using USRP based SDR platforms on the ORBIT testbed. Further, inter-network coordination with logically centralized radio resource management across Wi-Fi and LTE systems is proposed as a possible solution for improved co-existence. Numerical results are presented showing significant gains in both Wi-Fi and LTE performance with the proposed inter-network coordination approach.

==> motivation.tex <==
\section{Interference Characterization}
\label{sec:interChara}

\subsection{Interference Characterization Model}
\label{subsec:interChara}
We propose an analytical model to characterize the interference between Wi-Fi and LTE, while considering the Wi-Fi sensing mechanism (clear channel assessment (CCA)) and scheduled and persistent packet transmission at LTE. To illustrate, we focus on a co-channel deployment involving a single W-iFi and a single LTE cell, which involves disseminating the interaction of both technologies in detail and establish a building block to study a complex co-channel deployment of multiple Wi-Fis/LTEs.

In a downlink deployment scenario, a single client and a full buffer (saturated traffic condition) is assumed at each AP under no MIMO\footnotetext[1]{Throughput the paper, LTE home-eNB (HeNB) is also referred as access point (AP) for the purpose of convenience}. Transmit powers are denoted as $P^{i}, i\in\{w,l\}$ where $w$ and $l$ are indices to denote Wi-Fi and LTE, respectively. We note that the maximum transmission power of an LTE small cell is comparable to that of the Wi-Fi, and thus is consistent with regulations of unlicensed bands.

The power received from a transmitter $j$ at a receiver $i$ is given by $P_jG_{ij}$ where $G_{ij} \geq 0$ represents a channel gain which is inversely proportional to $d_{ij}^\gamma$ where $d_{ij}$ is the distance between $i$ and $j$ and $\gamma$ is the path loss exponent. $G_{ij}$ may also include antenna gain, cable loss, wall loss, and other factors. Signal-to-Interference-plus-Noise (SINR) on the link $i$ given as
\begin{equation}
\label{sinr}
S_i = \frac{P^iG_{ii}}{P_jG_{ij} + N_i}
\end{equation}
where $N_i$ is noise power for receiver $i$. Here, in the case of a single Wi-Fi and LTE, if $i$ represents the Wi-Fi link, then $j$ is the LTE link, and vice versa.

The throughput, $R^i, i\in\{w,l\}$, can be represented as a function of $S_i, i\in\{w,l\}$ as
\begin{equation}
\label{eq:dataRate}
R^i = \alpha^i B \log_2(1 + \beta^iS_i), \;\; i\in\{w,l\},
\end{equation}
where $B$ is a channel bandwidth; $\beta^i$ is a factor  associated with the modulation scheme. For LTE, $\alpha^l$ is a bandwidth efficiency of $i\in\{w,l\}$ due to factors adjacent channel leakage ratio and practical filter, cyclic prefix, pilot assisted channel estimation, signaling overhead, etc. For Wi-Fi, $\alpha^w$ is the bandwidth efficiency of CSMA/CA, which comes from the Markov chain analysis of CSMA/CA\cite{bianchi2000_802.11DCF} with
\begin{equation}
\label{eq:markov_chain}
\begin{aligned}
\eta_E = \frac{T_E}{\mathrm{E}[S]}, \;
\eta_S = \frac{T_S}{\mathrm{E}[S]}, \;
\eta_C = \frac{T_C}{\mathrm{E}[S]},
\end{aligned}
\end{equation}
where $\mathrm{E}[S]$ is the expected time per Wi-Fi packet transmission; $T_E$, $T_S$, $T_C$ are the average times per $\mathrm{E}[S]$ that the channel is empty due to random backoff, or busy due to the successful transmission or packet collision (in case of multiple Wi-Fis in the CSMA range), respectively. $\alpha^w$ is mainly associated with $\eta_S$.

In our analysis, $\{\alpha^i,\beta^i\}$ is approximated so that - (1) for LTE, $R^l$ matches with throughput achieved under variable channel quality index (CQI), and (2) for Wi-Fi, $R^w$ matches throughput achieved under Biachi's CSMA/CA model.

\subsubsection{Characterization of Wi-Fi Throughput}
Assuming CCA$_T$ is CCA threshold to detect channel as busy or not, if channel energy at the Wi-Fi node is higher than CCA$_T$, Wi-Fi would hold back the data transmission, otherwise it transmit at a data rate based on the SINR of the link. Wi-Fi throughput with and without LTE is given as~\\\\
\begingroup
\removelatexerror% Nullify \@latex@error
\IncMargin{2em}
\begin{algorithm}[H]
\DontPrintSemicolon
%\SetVline
\vspace{.3em}
\SetAlgoLined
\SetAlgorithmName{Model}{List of models};
\SetKwInOut{Output}{Output}
\SetKwInOut{Para}{Parameter}

\KwData{$P^w$: Wi-Fi Tx power; $G_w$: channel gain of Wi-Fi link; $P^l$: LTE Tx power; $G_{wl}$: channel gain(LTE AP, Wi-Fi UE); $N_0$: noise power; $E_c$: channel energy at the Wi-Fi (LTE interference + $N_0$).}
\Para{$\lambda_C$: Wi-Fi CCA threshold}
\Output{$R^w$: Wi-Fi throughput}
%\KwResult{how to write algorithm with \LaTeX2e }

\eIf{No LTE}{
\vspace{-0.5em}
\[\begin{aligned}
    R^w  = \alpha^w W \log_2\left(1 + \beta^w \frac{P^wG_w}{N_0}\right).
\end{aligned}\]
\vspace{-0.5em}
}
( When LTE is present){\eIf{$E_c >$ $\lambda_C$}{
No Wi-Fi transmission with $R^w = 0$
}{
\vspace{-0.5em}
\[\begin{aligned}
	R^w  = \alpha^w W \log_2\left(1 + \beta^w \frac{P^wG_w}{P^lG_{wl} + N_0}\right).
\end{aligned}\]
\vspace{-1em}
}}
\caption{Wi-Fi Throughput Characterization}
\end{algorithm}
\DecMargin{2em}
\endgroup


\subsubsection{Characterization of LTE Throughput}~
Due to CSMA/CA, Wi-Fi is active for an average $\eta_S$ fraction of time (Eq. \eqref{eq:markov_chain}). Assuming that LTE can instantaneously update its transmission rate based on the Wi-Fi interference, its throughput can be modeled as follows- ~\\\\
\begingroup
\removelatexerror% Nullify \@latex@error
\IncMargin{2em}
\begin{algorithm}[H]
\DontPrintSemicolon
\vspace{.3em}
\SetAlgoLined
\SetAlgorithmName{Model}{List of models};
\SetKwInOut{Output}{Output}
\SetKwInOut{Para}{Parameter}

\KwData{$P^l$: LTE Tx power; $G_l$: channel gain of LTE link; $P^w$: Wi-Fi Tx power; $G_{lw}$: channel gain(Wi-Fi AP,LTE UE); $N_0$: noise power; $E_c$: channel energy at Wi-Fi (LTE interference + $N_0$);}
\Para{$\lambda_C$: Wi-Fi CCA threshold}
\Output{$R^l$: LTE throughput}
%\KwResult{how to write algorithm with \LaTeX2e }

\eIf{No Wi-Fi}{
\vspace{-0.5em}
\[\begin{aligned}
    R^l_{\mbox{noW}}  &= \alpha^l W \log_2\left(1 + \beta^l \frac{P^lG_l}{N_0}\right).
\end{aligned}\]
\vspace{-0.5em}
}
( When Wi-Fi is present){\eIf{$E_c >$ $\lambda_C$}{
No Wi-Fi transmission/interference
\[\begin{aligned}
    R^l &= R^l_{\mbox{noW}}.
\end{aligned}\]
\vspace{-1.2em}
}{
\vspace{-0.5em}
\[\begin{aligned}
    R^l  &= \alpha^l W \log_2\left(1 + \beta^l \frac{P^lG_l}{P^lG_{lw} + N_0}\right).
\end{aligned}\]
Using \eqref{eq:markov_chain} and $\eta_C = 0$ (a single Wi-Fi)
\[\begin{aligned}
    R^l &= \eta_E R^l_{\mbox{noW}} +  \eta_S R^l
\end{aligned}\]
\vspace{-1.2em}
}}
\caption{LTE Throughput Characterization}
\end{algorithm}
\DecMargin{2em}
\endgroup

\begin{figure}[t]
\begin{center}
\includegraphics[height=1.5in,width=3in]{pics/scene1_interonWiFi.eps}
\caption{Experimental scenario to evaluate the throughput performance of Wi-Fi $w_1$ in the presence of interference (LTE/other Wi-Fi/white noise) when both $w_1$ and interference operated on the same channel in 2.4 GHz}
\label{fig:scene1_interonWiFi}
\end{center}
\vspace{-0.3cm}
\end{figure}

\begin{figure}[t]
\begin{center}
\includegraphics[height=2in,width=2.75in]{pics/compAnaModelvsExp_11g.eps}
\caption{Comparative results analytical model and experiments to show the effect of LTE on the throughput of Wi-Fi 802.11g  when distance between LTE eNB and Wi-Fi link is varied.}
\label{fig:compAnaModelvsExp_11g}
\end{center}
%\vspace{-0.3cm}
\end{figure}

\begin{figure}[t]
\begin{center}
\includegraphics[height=2in,width=2.75in]{pics/distvsThru_11g_MME.eps}
\caption{Comparative results analytical model and experiments to show the effect of LTE on the throughput of Wi-Fi 802.11g  when distance between LTE HeNB (AP) and Wi-Fi link is varied.}
\label{fig:distvsThru_11g_MME}
\end{center}
%\vspace{-0.1cm}
\end{figure}


\begin{table}[t]
\caption{Network parameters of Wi-Fi/LTE deployment}
\centering
\begin{tabular}{| l | l | l | l |}
\hline
\textbf{Parameter} & \textbf{Value} & \textbf{Parameter} & \textbf{Value}\\
\hline
Scenario & Downlink & Tx power & 20 dBm\\
\hline
Spectrum band & 2.4 GHz & Channel bandwidth & 20 MHz\\
\hline
Traffic model & \multicolumn{3}{|l|}{Full buffer via saturated UDP flows}\\
\hline
AP antenna height & 10 m & User antenna height & 1 m\\
\hline
Path loss model & \multicolumn{3}{|l|}{36.7$\log_{10}$(d[m]) + 22.7 + 26$\log_{10}$(frq [GHz])}\\
\hline
Noise Floor & \multicolumn{3}{|l|}{-101 dBm, (-174 cBm thermal noise/Hz)}\\
\hline
Channel & \multicolumn{3}{|l|}{No shadow/Rayleigh fading}\\
\hline
\end{tabular}
\label{tab:net_para}
%\vspace{-0.2cm}
\end{table}


\subsection{Experimental Validation}
In this section, we experimentally validate proposed interference characterization models using experiments involving the ORBIT testbed and USRP radio platforms available at WINLAB\cite{Ray2005_ORBITOverview,usrpB210}. An 802.11g Wi-Fi link is set up  using Atheros AR928X wireless network adapters\cite{ath9k} and an AP implementation with \textit{hostapd}\cite{hostapd}. For LTE, we use \textit{OpenAirInterface}, an open-source software implementation, which is fully compliant with 3GPP LTE standard (release 8.6) and set in transmission mode 1 (SISO)\cite{Nikaein2014_OAI}. Currently, \textit{OpenAirInterface} is in the development mode for USRP based platforms with limited working LTE operation parameters.

In our experiment, depicted as the scenario shown in figure~\ref{fig:scene1_interonWiFi}, we study the effect of interference on the Wi-Fi link $w_1$. For link $w_1$, the distance between the AP and client is fixed at $0.25$ m (very close so that the maximum throughput is guaranteed when interference is present. Experimentally, we observe maximum throughput as $22.2$ Mbps). The distance between the interfering AP and Wi-Fi AP is varied in the range of 1 to 20 m. The throughput of $w_1$ is evaluated under three sources of interference - LTE, Wi-Fi and white noise, when both $w_1$ and the interference AP is operated on the same channel in the 2.4 GHz spectrum band. These experiments are carried in the 20 m-by-20 m ORBIT room in WINLAB, which has an indoor Line-of-Sight (LoS) environment. For each source of interference, Wi-Fi throughput is averaged over 15 sets of experiments with variable source locations and trajectories between interference and $w_1$.

In the first experiment, we perform a comparison study to evaluate the effect of LTE interference on $w_1$, observed by experiments and computed by interference characterization model. In this case, LTE signal is lightly loaded on 5 MHz of bandwidth mainly consist of control signals. Thus, the impact of such LTE signal over the Wi-Fi band is equivalent to the low power LTE transmission. Thus, we incorporate these LTE parameters in our analytical model. As shown in figure~\ref{fig:compAnaModelvsExp_11g}, we observe that both experimental and analytical values match the trend very closely, though with some discrepancies. These discrepancies are mainly due to the fixed indoor experiment environment and lack of a large number of experimental data sets. Additionally, we note that even with the LTE control signal (without any scheduled LTE data transmission), performance of Wi-Fi gets impacted drastically.

In the next set of experiments, we study the throughput of a single Wi-Fi link in the presence of different sources of interference - (1) Wi-Fi, (2) LTE operating at 5 MHz, and (3) LTE operating at 10 MHz, evaluating each case individually. For this part, full-band occupied LTE is considered with the maximum power transmission of $100$ mW. As shown in figure~\ref{fig:distvsThru_11g_MME}, when the Wi-Fi link operates in the presence of other Wi-Fi links, they share channel according to the CSMA/CA protocol and throughput is reduced approximately by half. In the both the cases of LTE operating at 5 and 10 MHz, due to lack of coordination, Wi-Fi throughput gets impacted by maximum upto $90\%$ compared to no interference Wi-Fi throughput and $20-80\%$ compared to Wi-Fi thorughput in the presence of other Wi-Fi link. 
%Thus, these results emphasizes the need of coordination among these two technologies.
These results indicate significant inter-system interference in the baseline case without any coordination between systems. 

\subsection{Motivational Example}
\label{subsec:motiEx}
We extend our interference model to complex scenarios involving co-channel deployment of a single link Wi-Fi and LTE for the detailed performance evaluation. As shown in figure~\ref{fig:scene2_varIntAPUEdist}, UE$_i$, associated AP$_i$ and interfering AP$_j$, $i,j \in \{w,l\}, i \neq j$, are deployed in a horizontal alignment. The distance, $d_A$, between UE$_i$ and AP$_i$ is varied between $0$ and $100$ m. At each value of $d_A$, the distance between UE$_i$ and AP$_j$ is varied in the range of $-100$ to $100$ m. Assuming UE$_i$ is located at the origin $(0,0)$, if AP$_j$ is located on the negative X-axis then the distance is denoted as $-d_I$, otherwise as $+d_I$, where $d_I$ is an Euclidean norm $\|\text{UE}_i,\text{AP}_j\|$. In the shared band operation of Wi-Fi and LTE, due to the CCA sensing mechanism at the Wi-Fi node, the distance between Wi-Fi and LTE APs (under no shadow fading effect in this study) decides the transmission or shutting off of Wi-Fi. Thus, the above distance convention is adopted to embed the effect of distance between AP$_i$ and AP$_j$. Simulation parameters for this set of simulations are given in Table~\ref{tab:net_para}.

\begin{figure}[t]
\begin{center}
\includegraphics[height=1.5in,width=3.5in]{pics/scene2_varIntAPUEdist.eps}
\caption{Experimental scenario to evaluate the throughput performance of Wi-Fi $w_1$ in the presence of interference (LTE/other Wi-Fi/white noise) when both $w_1$ and interference operated on the same channel in 2.4 GHz}
\label{fig:scene2_varIntAPUEdist}
\end{center}
%\vspace{-0.3cm}
\end{figure}

\begin{figure}[t]
\centering
\subfigure[A heat map of Wi-Fi throughput (Mbps)]{
	\includegraphics[height=1.75in,width=2.3in]{pics/wthru_lteInter_3D.eps}
    \label{fig:wthru_lteInter_3D}
%	\vspace{-0.8cm}
}
\subfigure[Wi-Fi performance sections- High SINR: non-zero throughput, Low SINR: SINR below minimum SINR requirement, CCA$\_$busy: shutting off of Wi-Fi due to channel is sensed as busy]{
	\includegraphics[height=1.75in,width=2.3in]{pics/w_perfSections.eps}
    \label{fig:w_perfSections}
%	\vspace{-0.8cm}
}
\caption[Optional caption for list of figures]{Wi-Fi performance as a function of distance(Wi-Fi AP, associated Wi-Fi UE) $d_A$ and distance(Interfering LTE AP, Wi-Fi UE) $d_I$  %%\subref{fig:NvswoACAwACA}, \subref{fig:NvsACAgainRanFix}
}
\label{fig:wifi_noOpt}
%\vspace{-0.5cm}
\end{figure}

Figure~\ref{fig:wifi_noOpt} shows the Wi-Fi performance in the presence of LTE interference. As shown in figure~\ref{fig:wthru_lteInter_3D}, the Wi-Fi throughput is drastically deteriorated in the co-channel LTE operation, leading to zero throughput for $80\%$ of the cases and an average $91\%$ of throughput degradation compared to standalone operation of Wi-Fi. Such degradation is explained by figure~\ref{fig:w_perfSections}. Region \textit{CCA$\_$busy} shows the shutting off of the Wi-Fi AP due to the CCA mechanism, where high energy is sensed in the Wi-Fi band. This region corresponds to cases when Wi-Fi and LTE APs are within $\sim 20$m of each other. In the \textit{low SINR} region, the Wi-Fi link does not satisfy the minimum SINR requirement for data transmission, thus the Wi-Fi throughput is zero. \textit{High SINR} depicts the data transmission region that satisfies SINR and CCA requirements and throughput is varied based on variable data rate/SINR.


\begin{figure}[t]
\centering
\subfigure[A heat map of LTE throughput (Mbps)]{
	\includegraphics[height=1.75in,width=2.3in]{pics/Lthru_wifiInter_3D.eps}
    \label{fig:Lthru_lteInter_3D}
%	\vspace{-0.8cm}
}
\subfigure[LTE performance sections- High SINR: non-zero throughput, Low SINR: SINR below minimum SINR requirement, CCA$\_$busy: shutting off of Wi-Fi due to channel is sensed as busy]{
	\includegraphics[height=1.75in,width=2.3in]{pics/L_perfSections.eps}
    \label{fig:L_perfSections}
%	\vspace{-0.8cm}
}
\caption[Optional caption for list of figures]{LTE performance as a function of distance(LTE AP, associated LTE UE) $d_A$ and distance(Interfering Wi-Fi AP, LTE UE) $d_I$  %%\subref{fig:NvswoACAwACA}, \subref{fig:NvsACAgainRanFix}
}
\label{fig:lte_noOpt}
%\vspace{-0.5cm}
\end{figure}


On the other hand, figure~\ref{fig:lte_noOpt} depicts the LTE throughput in the presence of Wi-Fi interference.  LTE throughput is observed to be zero in the \textit{low SINR} regions, which is $45\%$ of the overall area and the average throughput degradation is $65\%$ compared to the standalone LTE operation. Under identical network parameters, overall performance degradation for LTE is much lower compared to that of Wi-Fi in the previous example. The reasoning for such a behavior discrepancy is explained with respect to figure~\ref{fig:L_perfSections} and the Wi-Fi CCA mechanism. In the \textit{CCA$\_$busy} region, Wi-Fi operation is shut off and LTE operates as if no Wi-Fi is present. In both LTE and the previous Wi-Fi examples, \textit{low SINR} represents the hidden node problem where two APs do not detect each other's presence and data transmission at an UE suffers greatly.




\eat{
\subsection{Experimental Setup}
In the literature, there are no previous studies experimentally evaluating the coexistence performance of LTE-Wi-Fi. In baseline experiment, the throughput performance of a Wi-Fi client varies as the BW and power level of the additive white Gaussian noise (AWGN) vary (refer figure \ref{fig:noiseBWvsThru}). This emphasize the necessity to characterize the impact of Wi-Fi and LTE on each other given various topologies, channel assignment, BW allocation etc. scenarios. For the experiment, we use the ORBIT testbed and USRP/GNU radio platforms available at WINLAB as shown in figure \ref{fig:orbitSet_noiseLTE}. Thus, we propose to apply the experimental characterization of LTE - Wi-Fi coexistence in the system level optimization given in eq.\ref{eq:optEq}.  Our goal is to obtain a set of LTE - Wi-Fi interference measurements that can be used to run the proposed optimization model and other alternatives to be developed in the future.

\begin{figure}[t]
\begin{center}
\includegraphics[height=2.2in,width=3in]{pics/distvsThru_11g.eps}
\caption{Effect of lightly loaded LTE on the throughput of Wi-Fi 802.11g  when distance between LTE eNB and Wi-Fi link is varied.}
\label{fig:distvsThru_11g}
\end{center}
%\vspace{-0.3cm}
\end{figure}


\begin{figure}[t]
\begin{center}
\includegraphics[height=2in,width=2.6in]{pics/orbitSet_noiseLTE.eps}
\caption{ORBIT experimental setup}
\label{fig:orbitSet_noiseLTE}
\end{center}
%\vspace{-0.3cm}
\end{figure}

\begin{figure}[t]
\begin{center}
\includegraphics[height=2.2in,width=3in]{pics/noiseBWvsThru_mobisysPPT.eps}
\caption{Performance of Wi-Fi as a function AWGN bandwidth overlapping and power level.}
\label{fig:noiseBWvsThru}
\end{center}
%\vspace{-0.3cm}
\end{figure}
} 

==> optimizationLTEWiFi.tex <==
\section{Coordination via Joint Optimization}
\label{sec:optimize}

\subsection{Joint Power Control Optimization}
Here, the objective is to optimize the set of transmission power $P^k_i,\forall i,k\in\{w,l\}$ at Wi-Fi and LTE APs, which maximizes the aggregated Wi-Fi+LTE throughput. Conventionally, LTE supports the power control in the cellular network. By default, commercially available Wi-Fi APs/routers are set to maximum level\cite{iw}. But adaptive power selection capability is incorporated in available 802.11a/g/n Wi-Fi drivers, even though it is not invoked very often. Under the SDN architecture, 
transmission power level can be made programmable to control the influence of interference from any AP at neighboring radio devices based on the spectrum parameters\cite{Gudipati2013_SoftRAN}.

For the maximization of aggregated throughput, we propose a geometric programming (GP) based power control\cite{Chiang2007_pwrCtr}. For the problem formulation, throughput, given by Eq.~\ref{eq:dataRate}, can approximated as
\begin{equation}
\label{eq:dataRate_1}
\begin{aligned}
R^k_i = \alpha^k \log_2(\beta^kS_i),
\end{aligned}
\end{equation}
where $i\in\{W,L\},k\in\{w,l\}$. This equation is valid when $\beta^iS_i$ is much higher than 1. In our case, this approximation is reasonable considering minimum SINR requirements for data transmission at both Wi-Fi and LTE. The aggregate throughput of the WiFi+LTE network is
\begin{equation}
\label{eq:dataRate_sys}
\begin{aligned}
\mathbb{R} &= \sum_{i\in W} a_i b_i \alpha^w \log_2(\beta^w S_i) + \sum_{j\in L} \alpha^l \log_2(\beta^l S_j)\\
&= \log_2\left[\left(\prod_{i\in W} (\beta^w S_i)^{a_i b_i \alpha^w} \right) \left(\prod_{j \in L} (\beta^l S_i)^{\alpha^l} \right)\right].
\end{aligned}
\end{equation}

In the coordinated framework, it is assumed that WiFi parameters $a_i$ and $b_i$ are updated periodically. Thus, these are considered as constant parameters in the formulation. Also, $\alpha^i, \beta^i, i\in\{w,l\}$ are constant in the network. Therefore, aggregate throughput maximization is equivalent to maximization of a product of SINR at both WiFi and LTE links. Power control optimization formulation is given by:
\begin{equation}
\begin{aligned}
& {\text{maximize}}
& & \left(\prod_{i\in W} (\beta^w S_i)^{a_i b_i \alpha^w} \right) \left(\prod_{j \in L} (\beta^l S_i)^{\alpha^l} \right)\\
& \text{subject to}
& & R^w_{i} \geq R^w_{i,\min}, \;\; \forall i\in W,\\
&&& R^l_{i} \geq R^l_{i,\min}, \;\; \forall i\in L,\\
&&& {\sum_{k\in M^b_i} P^w_{k}G_{ik}+\sum_{j\in L} P^l_{j}G_{ij}} + N_0 < \lambda_c, \; \forall i\in W,\\
&&& 0 < P^w_i \leq P_{\max}, \;\; \forall  i\in W,\\
&&& 0 < P^l_i \leq P_{\max}, \;\; \forall  i\in L.\\
\end{aligned}
\end{equation}

Here, the first and second constraints are equivalent to $S_i \geq S_{i,min}, \forall i$ which ensures that SINR at each link achieves a minimum SINR requirement, thus leading to non-zero throughput at the UE. The third constraint assures that channel energy at a WiFi (LTE interference + interference from WiFis in the interference zone + noise power) is below the clear channel assessment threshold $\lambda_c$, thus WiFi is not shut off. The fourth and fifth constraints follow the transmission power limits at each link. Unlike past power control optimization formulations for cellular networks, WiFi-LTE coexistence requires to meet the SINR requirement at a WiFi UE and, additionally, CCA threshold at a WiFi AP. 

To ensure the feasibility of the problem where all constrains are not satisfied, notably for WiFi links, we relax the minimum data requirement constraint for LTE links. In our case, we reduce the minimum data requirement to zero. This is equivalent to shutting off certain LTE links which cause undue interference to neighboring WiFi devices.

\subsection{Joint Time Division Channel Access Optimization}
The relaxation of minimum throughput constraint in the joint power control optimization leads to throughput deprivation at some LTE links. Thus, joint power control is not sufficient when system demands to have non-zero throughput at each UE. In such cases, we propose a time division channel access optimization framework where network of each RAT take turns to access the channel. Assuming network $i, i\in \{w,l\}$ access the channel for $\eta, eta \in [0,1],$ fraction of time, network $j, j\in\{w,l\},j\neq i,$ holds back the transmission and thus no interference occurs at $i$ from $j$. For remaining $1-\eta$ fraction of time, $j$ access the channel without any interference from $i$. This proposed approach can be seen as a subset of power assignment problem, where power levels at APs of network $i, i\in\{w,l\},$ is set to zero in their respective time slots. The implementation of the protocol is out of scope of this paper.

In this approach, our objective is to optimize $\eta$, the time division of channel access, such that it maximizes the minimum throughput across both WiFi and LTE networks. We propose the optimization in two steps -

\begin{figure*}[t]
\begin{center}
\subfigure[A heat map of WiFi throughput when joint power Coordination (Mbps)]{
	\includegraphics[height=1.75in,width=2.3in]{pics/W_wiL_pwrOpt_3d.eps}
    \label{fig:W_wiL_pwrOpt_3d}
	%\vspace{-0.8cm}
}
\subfigure[Feasibility region of joint power Coordination]{
	\includegraphics[height=1.75in,width=2.1in]{pics/w_PwrOpt_feasible.eps}
    \label{fig:w_opt_feasible}
	%\vspace{-0.8cm}
}
\subfigure[A heat map of WiFi throughput when time division channel access coordination (Mbps)]{
	\includegraphics[height=1.75in,width=2.3in]{pics/w_wiL_TDOpt_3d.eps}
    \label{fig:W_wiL_pwrTDOpt_3d}
	%\vspace{-0.8cm}
}
\caption[Optional caption for list of figures]{WiFi performance under joint WiFi and LTE power control optimization  %%\subref{fig:NvswoACAwACA}, \subref{fig:NvsACAgainRanFix}
}
\label{fig:wifi_Opt}
%\vspace{-0.5cm}
\end{center}
\end{figure*}

\begin{figure*}[t]
\begin{center}
\subfigure[A heat map of LTE throughput when joint power Coordination (Mbps)]{
	\includegraphics[height=1.75in,width=2.3in]{pics/L_wiL_pwrOpt_3d.eps}
    \label{fig:L_wiL_pwrOpt_3d}
	%\vspace{-0.8cm}
}
\subfigure[Feasibility region of joint power Coordination]{
	\includegraphics[height=1.75in,width=2.1in]{pics/L_PwrOpt_feasible.eps}
    \label{fig:L_opt_feasible}
	%\vspace{-0.8cm}
}
\subfigure[A heat map of LTE throughput when time division channel access coordination (Mbps)]{
	\includegraphics[height=1.75in,width=2.3in]{pics/L_wiL_TDOpt_3d.eps}
    \label{fig:L_wiL_pwrTDOpt_3d}
	%\vspace{-0.8cm}
}
\caption[Optional caption for list of figures]{WiFi performance under joint WiFi and LTE power control optimization  %%\subref{fig:NvswoACAwACA}, \subref{fig:NvsACAgainRanFix}
}
\label{fig:lte_Opt}
%\vspace{-0.5cm}
\end{center}
\end{figure*}

\subsubsection{Power control optimization across network of same RAT}
Based on the GP-formulation, the transmission power of the APs across the same network $i, i\in\{w,l\},$ are optimized such that
\begin{equation}
\begin{aligned}
& {\text{maximize}}
& & \sum_{i} R^w_i\\
& \text{subject to}
& & R^w_{i} \geq R^w_{i,\min}, \;\; i\in W\\
&&& 0 \leq P^w_i \leq P_{\max}, \;\; i\in W,\\
&&& {\sum_{k\in M^b_i} P^w_{k}G_{ik} + N_0} < \lambda_c, \; i\in W.\\
\end{aligned}
\end{equation}
and
\begin{equation}
\begin{aligned}
& {\text{maximize}}
& & \sum_{i} R^l_i\\
& \text{subject to}
& & R^l_{i} \geq R^l_{i,\min}, \;\; i\in L\\
&&& 0 \leq P^l_i \leq P_{\max}, \;\; i\in L.\\
\end{aligned}
\end{equation}
Here, the objective function is equivalent to maximizing the product of SINRs at the networks $i, i\in \{w,l\}$. The first and second constraints ensure that we meet the minimum SINR and transmission power limits requirements at all links $i$. In this formulation, SINR at WiFi and LTE respectively given as
\begin{equation}
\label{eq:timeSha_sinr}
\begin{aligned}
S^w_i =& \frac{P^w_iG_{ii}}{N_0},\;\; i\in W,\\
S^l_i =& \frac{P^l_iG_{ii}}{\sum_{j\in L, j \neq i}P^l_jG_{ij} + N_0},\;\; i\in L.
\end{aligned}
\end{equation}

\subsubsection{Joint time division channel access optimization}
This is the joint optimization across both WiFi and LTE networks which is formulated as given below
\begin{equation}
\begin{aligned}
& {\text{maximize}}
& & \min\left(R^w_{i\in W},R^l_{j\in L}\right)\\
& \text{subject to}
& & 0 \leq \eta \leq 1.\\
\end{aligned}
\end{equation}
\eat{\begin{equation}
\begin{aligned}
& {\text{maximize}}
& & \min\left(R^w_{i\in W},R^l_{j\in L}\right)\\
& \text{subject to}
& & \delta_1 \leq \frac{\sum_{i\in W}R^w_i}{\sum_{j\in L}R^l_j} \leq \delta_2,\\
&&& 0 \leq \eta \leq 1.\\
\end{aligned}
\end{equation}}
Here, throughput values at all WiFi and LTE nodes are considered as a constant, which is the output of the previous step. Time division channel access parameter $\eta$ is optimized so that it maximizes the minimum throughput across all UEs.


\eat{
\begin{itemize}
\item{$N \rightarrow$}
number of each WiFi and LTE links,
\item{$w, l \rightarrow$}
indices for the WiFi and LTE network, respectively;
\item{$W \rightarrow$}
the set of WiFi links
\item{$L \rightarrow$}
the set of LTE links
\item{$C^w \rightarrow$}
boolean matrix $C^w \in \{0,1\}^{N\times K}$ is the channel assignment matrix of WiFi where $C^w_{ik} = 1$ if WiFi $i$ operates on channel $k$, $C^w_{ik} = 0$ otherwise,
\item{$C^l \rightarrow$}
boolean matrix $C^l \in \{0,1\}^{N\times K}$ is the channel assignment matrix of LTE where $C^l_{ik} = 1$ if LTE $i$ operates on channel $k$, $C^l_{ik} = 0$ otherwise,
\item{$P^l_i \rightarrow$}
transmission power of LTE $i$, where $0 \leq P^l_i \leq P^l_{\max}$,
\item{$G_{ij} \rightarrow$}
channel gain between nodes $i$ and $j$,
\item{$N_0 \rightarrow$}
noise density of the channel,
\item{$\gamma^j_i \rightarrow$}
Signal-to-Interference-plus-Noise-Ratio (SINR) at $i$ of network $j \in {w,l}$,
\item{$M^a \rightarrow$}
boolean matrix $M^a \in \{0,1\}^{N\times N}$ represents WiFi CSMA matrix where $M^a_{ij} = 1$ if WiFi APs $i$ and $j$ are in CSMA range of each other, $M^a_{ij} = 0$ otherwise, (convention: $M^a_{ij} = 1, i = j$),
\item{$a_{i} \rightarrow$}
approximate reduction in channel access time fraction at WiFi $i$ due to sharing of channel with other WiFis in the CSMA range
which are on the same channel as $i$
\item{$M^b \rightarrow$}
boolean matrix $M^b \in \{0,1\}^{N\times N}$ represents WiFi interference matrix where $M^b_{ij} = 1$ if WiFi APs $i$ and $j$ are in interference range of each other, $M_{ij} = 0$ otherwise,
\item{$b_{i} \rightarrow$}
reduction in channel access time fraction due to hidden node interference (interference from APs outside the carrier sense but strong enough signal to affect ongoing transmission)
\item{$Z^j_i \rightarrow$}
throughput at $i$ of network $j \in {w,l}$,
\end{itemize}

Parameters are:
\begin{itemize}
\item{$\lambda_c \rightarrow$}
the clear channel assessment (CCA) threshold for WiFi,
\item{$P^w \rightarrow$}
transmission power of WiFi (fixed value),
\item{$\beta \rightarrow$}
$\beta \in [0,1]$ captures  the average effect of hidden node interference per interferer,
\item{$\eta_B \rightarrow$}
LTE bandwidth efficiency due to factors adjacent channel leakage ratio and practical filter, cyclic prefix, pilot assisted channel estimation, signaling overhead
\item{$\gamma^j_{\min} \rightarrow$}
Minimum SINR required for network $j \in {w,l}$,
\item{$\gamma^j_{\max} \rightarrow$}
Maximum SINR required for network $j \in {w,l}$,
\item{$P^l_{\max} \rightarrow$}
Maximum transmission power allowed for LTE,
\item{$\zeta_{\min},\zeta_{\max} \rightarrow$}
proportional fairness constants to balance WiFi and LTE throughput, ideally $\zeta_{\min} = \zeta_{\max} = 1$.
\end{itemize}

\textbf{Objective}: to maximize sum-throughput across WiFi and LTE network\\
\textbf{Controlling variables}: $C^w, C^l$ and $P^l_i, \forall i\in L$

\begin{equation}
\begin{aligned}
& {\text{maximize}}
& & \sum_{i\in W} Z^w_i + \sum_{j\in L} Z^l_j\\
& \text{subject to}
& & C^w_{ik} \in \{0,1\}, \;\; \forall i\in W,\\
&&& C^l_{ik} \in \{0,1\}, \;\; \forall i\in L,\\
&&& \sum_{k} C^w_{ik} = 1, \; \forall i\in W,\\
&&& \sum_{k} C^l_{ik} = 1, \; \forall i\in L,\\
&&& {\sum_{k}\sum_{j\in L} C^w_{ik} C^l_{jk} P^l_{j}G_{ij}} + N_0 < \lambda_c, \; \forall i\in W,\\
&&& \gamma^l_i = \frac{P^l_iG_{ii}}{\sum_{k}C^l_{ik}\left( \sum_{m\in L, i\neq m} C^l_{mk}P^l_m G_{im} + \sum_{n\in W} C^w_{nk}a_nP^w G_{in} \right) + N_0}, \;\; \forall i\in L,\\
&&& \gamma^w_i = \frac{G_{ii}P^w}{\sum_{k}\sum_{j\in L} C^w_{ik} C^l_{jk} P^l_j G_{ij} + N_0}, \;\; \forall i\in W,\\
&&& a_{i} = \frac{1}{\sum_{k}\sum_{j\in W} C^w_{ik} C^w_{jk} M^a_{ij}}, \;\;  \forall i\in W,\\
&&& b_i = \frac{1}{1+\beta\sum_{k}\sum_{j\in W} C^w_{ik} C^W_{jk} M^b_{ij}}, \;\;  \forall i\in W,\\
&&& Z^w_i = a_ib_if(\gamma^w_i), \; \forall i\in W;\\
&&& Z^l_i = \eta_B\log(1 + \gamma^l_i), \; \forall i\in L,\\
&&& \zeta_{\min} \leq \frac{\sum_{i\in W} Z^w_i}{\sum_{j\in L} Z^l_j} \leq \zeta_{\max}, \\
&&& \gamma^w_{\min} \leq \gamma^w_i \leq \gamma^w_{\max}, \;\; \forall i\in W,\\
&&& \gamma^l_{\min} \leq \gamma^l_i \leq \gamma^l_{\max}, \;\; \forall i\in L,\\
&&& 0 \leq P^l_i \leq P^l_{\max}, \;\; \forall  i\in L.\\
\end{aligned}
\end{equation}
}


==> sysModel.tex <==
\section{System Model}
\label{sec:sysModel}
As seen in the previous section, when two (or more) APs of different Wi-Fi and LTE networks are deployed in the same spectrum band, APs can cause severe interference to one another. In order to alleviate inter-network interference, we propose joint coordination based on (1) power, and (2) time division channel access optimization. We assume that both LTE and Wi-Fi share a single spectrum channel and operate on the same amount of bandwidth. We also note that clients associated to one AP cannot join other Wi-Fi or LTE APs. This is a typical scenario when multiple autonomous operators deploy APs in the shared band. With the help of the proposed SDN architecture, power level and time division channel access parameters are forwarded to each network based on the throughput requirement at each UE. To the best of our knowledge, such an optimization framework has not yet received much attention for the coordination between Wi-Fi and LTE networks.

We consider a system with $N$ Wi-Fi and $M$ LTE networks. $W$ and $L$ denote the sets of Wi-Fi and LTE links, respectively. We maintain all assumptions, definitions and notations as described in Section \ref{subsec:interChara}. For notational simplicity, we redefine $R^i = \alpha^i B \log_2(1 + \beta^i S_i)$ as $R^i = \alpha^i \log_2(1 + \beta^i S_i)$, where constant parameter $B$ is absorbed with $\alpha^i$. Additional notation are summarized in Table \ref{tab:optNot}.
\begin{table}[t]
\caption{Definition of notations}
\centering
\begin{tabular}{| l | l |}
\hline
\textbf{Notation} & \textbf{Definition}\\
\hline
$w, l$ & indices for Wi-Fi and LTE network, respectively\\
\hline
$W$ & the set of Wi-Fi links\\
\hline
$L$ & the set of LTE links \\
\hline
$P^i_j$ & Transmission power of $j$-th AP of $i,\in\{w,l\}$ \\
\hline
$G_{ij}$ & Channel gain between nodes $i$ and $j$ \\
\hline
$R^i_j$ & Throughput at $j$-th link of $i,\in\{w,l\}$ \\
\hline
$S^i_j$ & SINR at $j$-th link of $i,\in\{w,l\}$ \\
\hline
$B$ & Channel Bandwidth\\
\hline
$N_0$ & Noise level \\
\hline
$\alpha^i,\beta^i$ & Efficiency parameters of network $i\in\{w,l\}$\\
\hline
$M^a_i$ & Set of Wi-Fi APs in the CSMA range of AP $i$ \\
\hline
$M^b_i$ & Set of Wi-Fi APs in the interference range of AP $i$\\
\hline
$\zeta$ & Hidden node interference parameter\\
\hline
$\eta$ & Fraction of channel access time for network $i,i\in\{w,l\}$ when\\
& $j,j\in\{w,l\},j \neq i$, access channel for $1-\eta$ fraction of time\\
\hline
\end{tabular}
\label{tab:optNot}
%\vspace{-0.2cm}
\end{table}


In order to account for the co-channel deployment of multiple Wi-Fi networks, we assume that time is shared equally when multiple Wi-Fi APs are within CSMA range due to the Wi-Fi MAC layer. We denote the set of Wi-Fi APs within the CSMA range of AP$_i, \forall i$ as $M^a_i$ and those outside of carrier sense but within interference range as $M^b_i$. When AP$_i$ shares the channel with $|M^a_i|$ other APs, its share of the channel access time get reduced to approximately $1/(1 + |M^a_i|)$. Furthermore, $M^b_i$ signifies a set of potential hidden nodes for AP$_i, \forall i$. To capture the effect of hidden node interference from APs in the interference range, parameter $\zeta$ is introduced which lowers the channel access time and thus, the throughput. Average reduction in channel access time at AP$_i$ is $1/(1 + \zeta|M^b_i|)$ where $\zeta$ falls in the range $[0.2,0.6]$\cite{baid2012_netCoop}. Therefore, the effective Wi-Fi throughput can be written as

\begin{equation}
\label{eq:w_thru}
\begin{aligned}
R^w_i = a_i b_i \alpha^w \log_2(1 + \beta^w S^w_i), \;\; i\in W,\\
\text{with } a_i = \frac{1}{1 + |M^a_i|} \text{ and } b_i = \frac{1}{1 + \zeta|M^b_i|}.
\end{aligned}
\end{equation}
SINR of Wi-Fi link, $i, \forall i$, in the presence of LTE and no LTE is described as
\begin{equation}
\label{eq:w_sinr}
S^w_i = \left\{ \begin{aligned}
&\frac{P^w_iG_{ii}}{N_0}, && \text{if no LTE};\\
&\frac{P^w_iG_{ii}}{\sum_{j\in L}P^l_jG_{ij} + N_0}, && \text{if LTE},
\end{aligned}
\right.
\end{equation}

where the term $\sum_{j\in L}P^l_jG_{ij}$ is the interference from all LTE networks at a Wi-Fi link $i$.

The throughput definition of the LTE link $i, \forall i$ remains the same as in Section \ref{subsec:interChara}:
\[
R^l_i = \alpha^l \log_2(1 + \beta^l S_i).
\]
The SINR of the LTE link, $i, \forall i$, in the presence of Wi-Fi and no Wi-Fi is described as
\begin{equation}
\label{eq:l_sinr}
S^l_i = \left\{ \begin{aligned}
&\frac{P^l_iG_{ii}}{\sum_{j\in L, j \neq i}P^l_jG_{ij} + N_0}, \; \text{if no Wi-Fi};\\
&\frac{P^l_iG_{ii}}{\sum_{j\in L, j \neq i}P^l_jG_{ij} + \sum_{k\in W}a_kP^w_kG_{ik} + N_0},\; \text{if Wi-Fi},
\end{aligned}
\right.
\end{equation}

where terms $\sum_{j\in L, j \neq i}P^l_jG_{ij}$ and $\sum_{k\in W}a_kP^w_kG_{ik}$ signifies the interference contribution from other LTE links and Wi-Fi links. For the $k$-th Wi-Fi link, $\forall k$, the interference is reduced by a factor $a_k$ to capture the fact that the $k$-th Wi-Fi is active approximately for only $a_k$ fraction of time due to the CSMA/CA protocol at Wi-Fi.

For a given model, inter-network coordination is employed to assure a minimum throughput requirement, thus the guaranteed availability of the requested service at each UE. For this purpose, we have implemented our optimization in two stages as described in following subsections.
\eat{Using SDN architecture, transmission power of Wi-Fi and LTE can be dynamically changed based on the global visibility of network with respect to geographical placement of Wi-Fi/LTE nodes, interference pattern at nodes, throughput requirement at each UE/application, etc.}
